Catalogue of Spacetimes

The Catalogue of Spacetimes is a collection of four-dimensional Lorentzian spacetimes in the context of the General Theory of Relativity (GR). The aim of the catalogue is to give a quick reference for students who need some basic facts of the most well-known spacetimes in GR.

==> deSitterUniv.tex <==
% ******** Start of file deSitterUniv.tex *********
%
%  Copyright (c) 2009,2010 Thomas Mueller
%                          Universitaet Stuttgart, VISUS
%

%% --------------------------------------
%%  lemaitre-robinson form
%% --------------------------------------
\subsection{Lema\^{\i}tre--Robinson form}
The de-Sitter universe in the Lema\^{\i}tre--Robinson form reads
\metricEq{
  ds^2 = -c^2dt^2 + e^{2Ht}\left[dr^2 + r^2\left(d\vartheta^2 + \sin(\vartheta)^2d\varphi^2\right)\right],
}{deSitterRobLemaitre}
with Hubble's Parameter $H=\sqrt{\frac{\Lambda c^2}{3}}$, which is assumed here to be time-independent. \\
%The transformation between the two representations of the metric is given by
%\begin{subequations}
%\begin{alignat}{3}
%\tilde{r} &= \frac{r}{\sqrt{1-H^2r^2}}e^{-Ht}, &\qquad \tilde{t} &= t + \frac{1}{2H}\ln\left(1 - H^2r^2\right), \\
%d\tilde{r} &= \frac{He^{-Ht}}{\sqrt{1-H^2r^2}}\left(\frac{dr}{1-H^2r^2} - rdt\right), &\qquad d\tilde{t} &= dt - \frac{Hr}{1 - H^2r^2}dr
%\end{alignat}
%\end{subequations}
%with \hspace{1mm}$\tilde{ }$\hspace{1mm} marking the coordinates in the Lema\^{\i}tre-Robinson form.
This a special case of the first and second form of the Friedman-Robertson-Walker metric defined in Eqs. (\ref{eqM:FRW1}) and (\ref{eqM:FRW2}) with $R(t) = e^{Ht}$ 
and $k=0$. \\
%% -------------------- Christoffel symbols --------------------
\SecChristoffel
\begin{subequations}
\begin{alignat}{5}
\Gamma_{tr}^r &= H, &\qquad \Gamma_{t\vartheta}^\vartheta &= H, &\qquad \Gamma_{t\varphi}^\varphi &= H, \\
\Gamma_{rr}^t &= \frac{e^{2Ht}H}{c^2}, &\qquad \Gamma_{r\vartheta}^\vartheta &= \frac{1}{r}, &\qquad \Gamma_{r\varphi}^\varphi &= \frac{1}{r}, \\
\Gamma_{\vartheta\vartheta}^t &= \frac{e^{2Ht}r^2 H}{c^2}, &\qquad \Gamma_{\vartheta\vartheta}^r &= -r, &\qquad \Gamma_{\vartheta\varphi}^\varphi &= \cot(\vartheta), \\
\Gamma_{\varphi\varphi}^t &= \frac{e^{2Ht}r^2\sin^2(\theta)H}{c^2}, &\qquad \Gamma_{\varphi\varphi}^r &= -r\sin(\vartheta)^2, &\qquad \Gamma_{\varphi\varphi}^\vartheta &= -\sin(\vartheta)\cos(\vartheta).
\end{alignat}
\end{subequations}

%% -------------------- Riemann tensor --------------------
\SecRiemann
\begin{subequations}
\begin{alignat}{3}
  R_{trtr} &= -e^{2Ht}H^2, &\qquad R_{t\vartheta t\vartheta} &= -e^{2Ht}r^2H^2, \\ 
  R_{t\varphi t\varphi} &= -e^{2Ht}r^2\sin^2(\vartheta)H^2, &\qquad R_{r\vartheta r\vartheta} &= \frac{e^{4Ht}r^2H^2}{c^2}, \\
  R_{r\varphi r\varphi} &= \frac{e^{4Ht}r^2\sin^2(\vartheta)H^2}{c^2}, &\qquad R_{\vartheta\varphi\vartheta\varphi} &= \frac{e^{4Ht}r^4\sin^2(\vartheta)H^2}{c^2} .
\end{alignat}
\end{subequations}

%% -------------------- Ricci tensor --------------------
\SecRicci
\begin{equation}
  R_{tt} = -3H^2,\qquad R_{rr} = 3\frac{e^{2Ht}H^2}{c^2}, \qquad R_{\vartheta\vartheta} = 3\frac{e^{2Ht}r^2H^2}{c^2},\qquad R_{\varphi\varphi} = 3\frac{e^{2Ht}r^2\sin^2(\vartheta)H^2}{c^2}.
\end{equation}

\noindent The {\sl Ricci scalar and Kretschman scalar read:}
\begin{equation}
  \mathcal{R} = \frac{12H^2}{c^2},\qquad \mathcal{K}=\frac{24H^4}{c^4}.
\end{equation}

%% -------------------- Local tetrad --------------------
\SecLocal
\begin{equation}
  \mathbf{e}_{(t)} = \frac{1}{c}\partial_{t}, \qquad \mathbf{e}_{(r)} = e^{-Ht}\partial_{r}, \qquad \mathbf{e}_{(\vartheta)} = \frac{e^{-Ht}}{r}\partial_{\vartheta}, \qquad \mathbf{e}_{(\varphi)} = \frac{e^{-Ht}}{r\sin{\vartheta}}\partial_{\varphi}.
\end{equation}

%% -------------------- Ricci rotation coefficients --------------------
\SecRicRotCoef
\begin{subequations}
\begin{align}
  \gamma_{(r)(t)(r)} &= \gamma_{(\vartheta)(t)(\vartheta)} = \gamma_{(\varphi)(t)(\varphi)} = \frac{H}{c} \\
  \gamma_{(\vartheta)(r)(\vartheta)} &= \gamma_{(\varphi)(r)(\varphi)} = \frac{1}{e^{Ht}r}, \quad\gamma_{(\varphi)(\vartheta)(\varphi)} = \frac{\cot(\theta)}{e^{Ht}r} .
\end{align}
\end{subequations}
The contractions of the Ricci rotation coefficients read
\begin{equation}
  \gamma_{(t)} = 3\frac{H}{c}, \qquad\gamma_{(r)} = \frac{2}{e^{Ht}r}, \gamma_{(\vartheta)} = \frac{\cot(\theta)}{e^{Ht}r}.
\end{equation}

%% -------------------- Riemann tensor LT--------------------
\SecRiemannLT
\begin{subequations}
\begin{align}
   R_{(t)(r)(t)(r)} &= R_{(t)(\vartheta)(t)(\vartheta)} = R_{(t)(\varphi)(t)(\varphi)} = -\frac{H^2}{c^2} \\
   R_{(r)(\vartheta)(r)(\vartheta)} &= R_{(r)(\varphi)(r)(\varphi)} = R_{(\vartheta)(\varphi)(\vartheta)(\varphi)} = \frac{H^2}{c^2}.
\end{align}
\end{subequations}

%% -------------------- Ricci tensor LT--------------------
\SecRicciLT
\begin{equation} 
  -R_{(t)(t)} = R_{(r)(r)} = R_{(\vartheta)(\vartheta)} = R_{(\varphi)(\varphi)} = 3\frac{H^2}{c^2}.
\end{equation}

%% ------------------------------------------------------
%%    Cartesian coordinates
%% ------------------------------------------------------
\subsection{Cartesian coordinates}
The de-Sitter universe can also be expressed using Cartesian coordinates:
\metricEq{
  ds^2 = -c^2dt^2 + e^{2Ht}\left[dx^2 + dy^2 + dz^2\right].
}{deSitterRobLemaitreCart}

%% -------------------- Christoffel symbols --------------------
\SecChristoffel
\begin{subequations}
\begin{alignat}{5}
\Gamma_{tx}^x &= H, &\qquad \Gamma_{ty}^y &= H, &\qquad \Gamma_{tz}^z &= H, \\
\Gamma_{xx}^t &= \frac{e^{2Ht}H}{c^2}, &\qquad \Gamma_{yy}^t &= \frac{e^{2Ht}H}{c^2}, &\qquad \Gamma_{zz}^t &= \frac{e^{2Ht}H}{c^2}. \\
\end{alignat}
\end{subequations}

Partial derivatives
\begin{equation}
  \Gamma_{xx,t}^t = \Gamma_{yy,t}^t = \Gamma_{zz,t}^t = \frac{2H^2e^{2Ht}}{c^2}.
\end{equation}

%% -------------------- Riemann tensor --------------------
\SecRiemann
\begin{subequations}
\begin{align}
  R_{txtx} &= R_{txtx} = R_{tztz} = -e^{2Ht}H^2, \\ 
  R_{xyxy} &= R_{xzxz} = R_{yzyz} = \frac{e^{4Ht}H^2}{c^2}. \\ 
\end{align}
\end{subequations}

%% -------------------- Ricci tensor --------------------
\SecRicci
\begin{equation}
  R_{tt} = -3H^2,\qquad R_{xx} = R_{yy} = R_{zz} = 3\frac{e^{2Ht}H^2}{c^2}.
\end{equation}

\noindent The Ricci and Kretschman scalar read:
\begin{equation}
  \mathcal{R} = 12\frac{H^2}{c^2},\qquad \mathcal{K}=24\frac{H^4}{c^4}.
\end{equation}

%% -------------------- Local tetrad --------------------
\SecLocal
\begin{equation}
  \mathbf{e}_{(t)} = \frac{1}{c}\partial_{t}, \qquad \mathbf{e}_{(x)} = e^{-Ht}\partial_{x}, \qquad \mathbf{e}_{(y)} = e^{-Ht}\partial_{y}, \qquad \mathbf{e}_{(z)} = e^{-Ht}\partial_{z}.
\end{equation}

%% -------------------- Ricci rotation coefficients --------------------
\SecRicRotCoef
\begin{equation}
  \gamma_{(x)(t)(x)} = \gamma_{(y)(t)(y)} = \gamma_{(z)(t)(z)} = \frac{H}{c}.
\end{equation}
The only non-vanishing contraction of the Ricci rotation coefficients read
\begin{equation}
  \gamma_{(t)} = 3\frac{H}{c}.
\end{equation}

%% -------------------- Riemann tensor LT--------------------
\SecRiemannLT
\begin{subequations}
\begin{align}
   R_{(t)(x)(t)(x)} &= R_{(t)(y)(t)(y)} = R_{(t)(z)(t)(z)} = -\frac{H^2}{c^2}, \\
   R_{(x)(y)(x)(y)} &= R_{(x)(z)(x)(z)} = R_{(y)(z)(y)(z)} = \frac{H^2}{c^2}.
\end{align}
\end{subequations}

%% -------------------- Ricci tensor LT--------------------
\SecRicciLT
\begin{equation} 
  -R_{(t)(t)} = R_{(x)(x)} = R_{(y)(y)} = R_{(z)(z)} = 3\frac{H^2}{c^2}.
\end{equation}

%% ------------------------------------------------------
%%
%% ------------------------------------------------------
%\subsection{Embedded in five-dimensional Euclidean space}
%Using the transformation 
%\begin{equation}
%\begin{aligned}
% \alpha &= r\sin(\vartheta)\cos(\varphi), &\qquad\beta &= r\sin(\vartheta)\sin(\varphi), &\qquad \gamma &= r\cos(\vartheta) \\ 
% \delta &= R\sqrt{1-\frac{r^2}{R^2}}\cosh(\nicefrac{t}{R}), &\qquad\varepsilon &= R\sqrt{1-\frac{r^2}{R^2}}\sinh(\nicefrac{t}{R}).
%\end{aligned}
%\end{equation}
%or
%\begin{equation}
%  \delta + \varepsilon = Re^{\nicefrac{t}{R}}\sqrt{1-\frac{r^2}{R^2}}, \qquad \delta - \varepsilon = Re^{-\nicefrac{t}{R}}\sqrt{1-\frac{r^2}{R^2}}.
%\end{equation}
%respectively, the de-Sitter spacetime can be changed into the form
%\begin{equation}
% ds^2 = -d\alpha^2 - d\beta^2 - d\gamma^2 - d\delta^2 + d\varepsilon^2
%\end{equation}
%now transforming according to
%\begin{equation}
% z_{1} = i\alpha, \qquad z_{2} = i\beta, \qquad z_{3} = i\gamma, \qquad z_{4} = i\delta, \qquad z_{5} = \varepsilon
%\end{equation}
%leads finally to
%\begin{equation}
% ds^2 = dz_{1}^2 + dz_{2}^2 + dz_{3}^2 + dz_{4}^2 + dz_{5}^2
%\end{equation}
%with the constraint
%\begin{equation}
% z_{1}^2 + z_{2}^2 + z_{3}^2 + z_{4}^2 + z_{5}^2 = -R^2
%\end{equation}
%which describes the de-Sitter spacetime as a 4-dimensional sphere embedded in 5-dimensional Euclidean space.

